Theory for the FCC-ee : Report on the 11th FCC-ee Workshop

The Future Circular Collider (FCC) at CERN, a proposed 100-km circular facility with several colliders in succession, culminates with a 100 TeV proton-proton collider. It offers a vast new domain of exploration in particle physics, with orders of magnitude advances in terms of Precision, Sensitivity and Energy. The implementation plan foresees, as a first step, an Electroweak Factory electron-positron collider. This high luminosity facility, operating between 90 and 365 GeV centre-of-mass energy, will study the heavy particles of the Standard Model, Z, W, Higgs, and top with unprecedented accuracy. The Electroweak Factory $e^+e^-$ collider constitutes a real challenge to the theory and to precision calculations, triggering the need for the development of new mathematical methods and software tools. A first workshop in 2018 had focused on the first FCC-ee stage, the Tera-Z, and confronted the theoretical status of precision Standard Model calculations on the Z-boson resonance to the experimental demands. The second workshop in January 2019, which is reported here, extended the scope to the next stages, with the production of W-bosons (FCC-ee-W), the Higgs boson (FCC-ee-H) and top quarks (FCC-ee-tt). In particular, the theoretical precision in the determination of the crucial input parameters, alpha_QED, alpha_QCD, M_W, m_t at the level of FCC-ee requirements is thoroughly discussed. The requirements on Standard Model theory calculations were spelled out, so as to meet the demanding accuracy of the FCC-ee experimental potential. The discussion of innovative methods and tools for multi-loop calculations was deepened. Furthermore, phenomenological analyses beyond the Standard Model were discussed, in particular the effective theory approaches. The reports of 2018 and 2019 serve as white papers of the workshop results and subsequent developments.

==> Headers/abstract.tex <==
%\vspace*{20mm}

%\centerline{\bf \Large Abstract}
\vspace*{12mm}
\noindent

{\small

The Future Circular Collider (FCC) at CERN, a proposed 100-km circular facility with several colliders in succession, culminates with a 100 TeV proton-proton collider. It offers a vast new domain of exploration in particle physics, with orders of magnitude advances in terms of precision, sensitivity and energy. The implementation plan published in 2018 foresees, as a first step, an Electroweak Factory electron-positron collider. This high luminosity facility, operating between 90 and 365 GeV centre-of-mass energy, will study the heavy particles of the Standard Model, Z, W, Higgs, and top with unprecedented accuracy. 
The physics programme offers great discovery potential:
(i) through exquisite precision measurements, 
(ii) through sensitive searches for symmetry violations, forbidden or extremely rare decays,  
and (iii) through the search for direct observation of new particles with extremely small couplings. 
The Electroweak Factory $e^+e^-$ collider
constitutes a real challenge to the theory and to precision calculations,  triggering the need for the development of new mathematical methods and software tools. 
A first workshop in 2018 had focused on the first FCC-ee stage, the Tera-Z, and confronted the theoretical status of precision 
Standard Model calculations on the $Z$-boson resonance to the experimental demands.  \\ 
\par
The second workshop in January 2019 extended the scope to the  next stages, with the production of W-bosons (FCC-ee-W), the Higgs boson (FCC-ee-H) and top quarks (FCC-ee-tt). 
In particular, the  theoretical precision in the  determination of the crucial input parameters,  $\alpha_{\mathrm{QED}}$,  $\alpha_{\mathrm{QCD}}$, $M_W$, $m_t$ at the level of FCC-ee requirements is thoroughly discussed. 
The requirements on Standard Model theory calculations were spelled out, so as to meet the demanding accuracy of the FCC-ee experimental potential.  
The discussion of innovative methods and tools for multi-loop calculations was deepened.
Furthermore, phenomenological analyses beyond the Standard Model  were discussed, in particular the effective theory approaches.
%{\color{blue} 
The reports of 2018 and 2019 serve as white papers of the workshop results and subsequent developments. 
}
%}

 

==> Headers/authors-carloni.tex <==
\begin{center}
A.~Blondel$^{1}$, ~J.~Gluza\footnote{Corresponding editor, email: janusz.gluza@cern.ch}$^{,2,3}$,  ~S.~Jadach$^4$, ~P.~Janot$^{5}$, ~T.~Riemann$^{2,6}$ (eds.),
\\
S.~Abreu$^{7}$, ~J.J.~Aguilera-Verdugo$^{8}$,
~A.B.~Arbuzov$^{9}$,
~J.~Baglio$^{10}$, ~S.D.~Bakshi$^{11}$, ~S.~Banerjee$^{12}$,
~M.~Beneke$^{13}$,
~C.~Bobeth$^{13}$, ~C.~Bogner$^{14}$,
~S.G.~Bondarenko$^{9}$,
~S.~Borowka$^{5}$, ~S.~Bra{\ss}$^{15}$, ~C.M.~Carloni~Calame$^{16}$,
~J.~Chakrabortty$^{11}$ ,
~M.~Chiesa$^{17}$,
~M.~Chrzaszcz$^{4}$, ~D.~d'Enterria$^{5}$,
~F.~Domingo$^{18}$, ~J.~Dormans$^{19}$,
~F.~Driencourt-Mangin$^{8}$,
~Ya.V.~Dydyshka$^{20}$,  ~J.~Erler$^{21,22}$,
~F.~Febres~Cordero$^{19,23}$, ~J.A.~Gracey$^{24}$, ~Zhi-Guo~He$^{25}$, ~G.~Heinrich$^{26}$, ~S.~Heinemeyer$^{27,28,29}$,
~I.~H\"onemann$^{14}$, ~H.~Ita$^{19}$, ~S.~Jahn$^{26}$, ~F.~Jegerlehner$^{6,30}$, ~S.P.~Jones$^{5}$,
~L.V.~Kalinovskaya$^{20}$,
~A.~Kardos$^{31}$, ~M.~Kerner$^{32}$, ~W.~Kilian$^{15}$,
~S.~Kluth$^{26}$, ~B.A.~Kniehl$^{25}$, ~A.~Maier$^{6}$,
~P.~Maierh\"ofer$^{19}$,
~G.~Montagna$^{33,16}$, ~O.~Nicrosini$^{16}$,
~T.~Ohl$^{17}$, ~B.~Page$^{34}$, ~S.~Pa{\ss}ehr$^{35}$,
~S.K.~Patra$^{11}$,  ~R.~Pittau$^{36}$, ~F.~Piccinini$^{16}$,
~W.~Placzek$^{37}$, ~J.~Plenter$^{8}$, ~S.~Ram\'{\i}rez-Uribe$^{8}$, 
~J.~Reuter$^{38}$, ~G.~Rodrigo$^{8}$, ~V.~Rothe$^{38}$,
~L.A.~Rumyantsev$^{20,39}$,
~R.R.~Sadykov$^{20}$,
~J.~Schlenk$^{40}$, ~G.F.R.~Sborlini$^{8}$, ~M.~Schott$^{21}$, ~A.~Schweitzer$^{41}$, ~C.~Schwinn$^{42}$, ~M.~Skrzypek$^{4}$, ~G.~Somogyi$^{43}$, ~M.~Spira$^{44}$, ~P.~Stienemeier$^{38}$, ~R.~Szafron$^{13}$, 
~K.~Tempest$^{45}$, ~W.J.~Torres Bobadilla$^{8}$, ~S.~Tracz$^{8}$, ~Z.~Tr\'ocs\'anyi$^{43,46}$, ~Z.~Tulip\'ant$^{43}$,
~J.~Usovitsch$^{47}$, ~A.~Verbytskyi$^{26}$, ~B.F.L.~Ward$^{48}$,
~Z.~Was$^{4}$, ~G.~Weiglein$^{38}$, ~C.~Weiland$^{49}$, ~S.~Weinzierl$^{21}$,
~V.L.~Yermolchyk$^{20}$
~S.A.~Yost$^{50}$, ~J.~Zurita$^{51,52}$

%\vspace*{1mm}  %tr 14 mm

\begin{flushleft}
{\em\small
{$^{1}$ 
DPNC, University of Geneva, Switzerland}
%DPNC, University of Geneva
\\
{$^2$ Institute  of Physics, University of Silesia, Katowice, Poland}
\\
{$^{3}$ Faculty of Science, University of Hradec Kr\'alov\'e, Czech Republic}
\\
{$^4$ Institute of Nuclear Physics, PAN, 
%ul. Radzikowskiego 152, 
31-342 Krak\'ow, Poland}
\\
{$^{5}$ CERN, CH-1211 Geneva 23, Switzerland}
\\
{$^{6}$ Deutsches Elektronen--Synchrotron, DESY, 15738 Zeuthen, Germany}
\\
{$^{7}$ Center for Cosmology, 
%Particle Physics and Phenomenology (CP3), 
CP3, 
Universit\'e Catholique de Louvain, 1348 Louvain-La-Neuve, Belgium}
\\
{$^{8}$ 
IFIC,
%Instituto de F\'{\i}sica Corpuscular, 
Universitat de Val\`{e}ncia,
% -- Consejo Superior de Investigaciones Cient\'{\i}ficas, 
%Parc Cient\'{\i}fic, 
E-46980 Paterna, Valencia, Spain}
\\
{$^{9}$ Bogoliubov Laboratory of Theoretical Physics, JINR, Dubna, 141980 Russia}
\\
{$^{10}$ Institut f\"ur Theoretische Physik, Eberhard Karls Universit\"at, 
%T\"ubingen, 
%Auf der Morgenstelle 14, 
72076 T\"ubingen, Germany}
\\
{$^{11}$ Indian Institute of Technology, Kanpur, India}
\\
{$^{12}$  University of Louisville, Louisville, KY 40292, USA}
 %        University of Louisville, Louisville, KY 40292 USA
\\
{$^{13}$ Physik Department T31, Technische Universit\"at M\"unchen, Garching, Germany}
\\
{$^{14}$ Institut f{\"u}r Physik, Johannes Gutenberg-Universit{\"a}t Mainz, D-55099 Mainz, Germany}
\\
{$^{15}$ Department Physik, Universit\"at Siegen, 
%Walter-Flex-Str. 3, 
57068 Siegen Germany}
\\
{$^{16}$ Istituto Nazionale di Fisica Nucleare, Sezione di Pavia, 
% via A. Bassi 6, 
27100 Pavia, Italy}
\\
{$^{17}$ Fakult\"at f\"ur Physik und Astronomie, Universit\"at W\"urzburg, 
% Emil-Hilb-Weg 22, 
97074 W\"urzburg Germany}
\\
{$^{18}$ Bethe Center for Theoretical Physics \& Physikalisches Institut der Universit\"at Bonn, 
%Nu{\ss}allee 12, 
53115 Bonn, Germany}
\\
{$^{19}$ Physikalisches Institut, Albert-Ludwigs-Universit\"at Freiburg, % Hermann-Herder-Str. 3, D-
79104 Freiburg, Germany}
\\
{$^{20}$  Dzhelepov Laboratory of Nuclear Problems, JINR, Dubna, 141980 Russia}
\\
{$^{21}$ PRISMA Cluster of Excellence, Inst. f{\"u}r Physik, Johannes Gutenberg-Universit{\"a}t, 55099 Mainz, Germany}
\\
{$^{22}$ 
        Departamento de F\'isica Te\'orica, Instituto de F\'isica, Universidad Nacional Aut\'onoma de M\'exico, 04510 CDMX, M\'exico}
\\
{$^{23}$ Physics Department, Florida State University, 
% 77 Chieftan Way, 
Tallahassee, FL 32306, U.S.A.}
\\
{$^{24}$ Theoretical Physics Division, 
        Department of Mathematical Sciences, University of Liverpool, 
        % P.O. Box 147, 
        Liverpool, L69 3BX, United Kingdom}
\\
{$^{25}$Institut f\"ur Theoretische Physik, Universit\"at Hamburg,
        % Luruper Chaussee 149, 
        22761 Hamburg, Germany}
\\
{$^{26}$ Max Planck Institute for Physics, 
% F\"ohringer Ring 6, 
80805 M\"unchen, Germany}
\\
{$^{27}$ Instituto de F\'isica Te\'orica (UAM/CSIC), Universidad Aut\'onoma de Madrid, Cantoblanco, 28049 Madrid, Spain}
\\
{$^{28}$ Instituto de F\'isica de Cantabria (CSIC-UC), 39005 Santander, Spain}
\\
{$^{29}$ Campus of International Excellence UAM+CSIC, Cantoblanco, 28049, Madrid, Spain}
\\
{$^{30}$ Institut f\"ur Physik, Humboldt--Universit\"at zu Berlin, 
% Newtonstrasse 15, D--
12489 Berlin, Germany}
\\
{$^{31}$Institute of Physics, University of Debrecen, 4010 Debrecen, 
% PO Box 105, 
Hungary},
\\
{$^{32}$ Physik-Institut, Universit{\"a}t Z{\"u}rich, % Winterthurerstrasse 190, 
8057 Z{\"u}rich, Switzerland}
\\
{$^{33}$ Dipartimento di Fisica, Universit\`a di Pavia, 
% via A. Bassi 6, 
27100 Pavia, Italy}
\\
{$^{34}$ Institut de Physique Th\'eorique, CEA, CNRS, Universit\'e Paris-Saclay, F-91191 Gif-sur-Yvette cedex, France}
\\
{$^{35}$ Sorbonne Universit\'e, CNRS, Laboratoire de Physique Th\'eorique et Hautes \'Energies (LPTHE), 
% 4 Place Jussieu, 
75252 Paris CEDEX 05, France}
\\
{$^{36}$ Departamento de F\'{i}sica Te\'orica y del Cosmos and CAFPE, Universidad de Granada, 
%Campus Fuentenueva s.n., E-
18071 Granada, Spain}
\\
{$^{37}$ Marian Smoluchowski Institute of Physics, Jagiellonian University, Cracow, Poland}
\\
{$^{38}$ Deutsches Elektronen--Synchrotron, DESY, 
% Notkestra{\ss}e 85, 
22607 Hamburg, Germany}
\\
{$^{39}$ Institute of Physics, Southern Federal University, Rostov-on-Don, 344090 Russia} 
\\
{$^{40}$ Institute for Particle Physics Phenomenology, University of Durham, Durham DH1 3LE, UK}
\\
{$^{41}$ Institute for Theoretical Physics, ETH Z\"urich, 
% Wolfgang-Pauli-Str. 27, 
8093 Z\"urich, Switzerland}
\\
{$^{42}$ Institut f\"ur Theoretische Teilchenphysik und   
        Kosmologie,   RWTH Aachen University, 
        % Sommerfeldstra\ss e 16,  
        52056 Aachen, Germany}
\\
{$^{43}$ MTA-DE Particle Physics Research Group, University of Debrecen, 4010 Debrecen, 
% PO Box 105, 
Hungary}
\\
{$^{44}$ Paul Scherrer Institut, CH-5232 Villigen PSI, Switzerland}
\\
{$^{45}$ Department of Physics, University of Toronto, 
% 60 St George St., 
Toronto, Ontario, M5S 1A7, Canada}
\\
{$^{46}$ Institute for Theoretical Physics, E\"otv\"os Lor\'and University, 
% P\'azm\'any P\'eter 1/A, H-
1117 Budapest, Hungary}
\\
{$^{47}$  School of Mathematics,
        Trinity College Dublin, The University of Dublin, Ireland}
\\
{$^{48}$ Baylor University, Waco, TX, USA}
\\
{$^{49}$ Pittsburgh Particle physics, Astrophysics, and Cosmology Center, Department of Physics and Astronomy, University of Pittsburgh,
% 3941 O'Hara St., 
Pittsburgh, PA 15260, USA}
\\
{$^{50}$ The Citadel, Charleston, SC, USA}
\\
{$^{51}$ Institute for Nuclear Physics (IKP), Karlsruhe Institute of Technology,
  % Hermann-von-Helmholtz-Platz 1, D-
  76344 Eggenstein-Leopoldshafen, Germany}
\\
{$^{52}$ Institute for Theoretical Particle Physics (TTP), Karlsruhe Institute of Technology, 
% Engesserstra\ss e 7, D-
76128 Karlsruhe, Germany}
}
\end{flushleft}
\end{center}

%before sanc authors
%\begin{center}
%A.~Blondel$^{1}$, ~J.~Gluza\footnote{Corresponding editor, E-mail: janusz.gluza@cern.ch}$^{,2,3}$,  ~S.~Jadach$^4$, ~P.~Janot$^{5}$, ~M.~McCullough$^{5}$, ~T.~Riemann$^{2,6}$ (eds.),
%\\
%S.~Abreu$^{7}$, ~J.J.~Aguilera-Verdugo$^{8}$, ~J.~Baglio$^{9}$, ~S.D.~Bakshi$^{10}$, ~S.~Banerjee$^{11}$, ~C.~Bobeth$^{12}$, ~C.~Bogner$^{13}$, ~S.~Borowka$^{5}$, ~S.~Bra{\ss}$^{14}$, ~J.~Chakrabortty$^{10}$ , ~M.~Chrzaszcz$^4$, ~F.~Domingo$^{15}$, ~J.~Dormans$^{16}$, ~F.~Driencourt-Mangin$^{8}$, ~F.~Febres~Cordero$^{16,17}$, ~J.A.~Gracey$^{18}$, ~Zhi-Guo~He$^{19}$, ~G.~Heinrich$^{20}$, ~S.~Heinemeyer$^{21,22,23}$,
%~I.~H\"onemann$^{13}$, ~H.~Ita$^{16}$, ~S.~Jahn$^{20}$, ~F.~Jegerlehner$^{6,24}$, ~S.~P.~Jones$^{5}$, ~A.~Kardos$^{25}$, ~M.~Kerner$^{26}$, ~W.~Kilian$^{14}$,
%~S.~Kluth$^{20}$, ~B.~A.~Kniehl$^{19}$, ~A.~Maier$^{6}$, ~P.~Maierh\"ofer$^{16}$, ~T.~Ohl$^{27}$, ~B.~Page$^{28}$, ~S.~Pa{\ss}ehr$^{29}$, ~S.K.~Patra$^{10}$, ~W.~Placzek$^{30}$, ~R.~Pittau$^{31}$, ~J.~Plenter$^{8}$, ~S.~Ram\'{\i}rez-Uribe$^{8}$, 
%~J.~Reuter$^{32}$, ~G.~Rodrigo$^{8}$, ~V.~Rothe$^{32}$, ~J.~Schlenk$^{33}$, ~G.~F.~R.~Sborlini$^{8}$, ~A.~Schweitzer$^{34}$, ~C.~Schwinn$^{35}$, ~M.~Skrzypek$^{4}$, ~G.~Somogyi$^{36}$, ~M.~Spira$^{37}$, ~P.~Stienemeier$^{32}$, ~R.~Szafron$^{12}$, 
%~K.~Tempest$^{38}$, ~W.~J.~Torres Bobadilla$^{8}$, ~S.~Tracz$^{8}$, ~Z.~Tr\'ocs\'anyi$^{37,39}$, ~Z.~Tulip\'ant$^{36}$,
%~J.~Usovitsch$^{40}$, ~A.~Verbytskyi$^{20}$, ~B.F.L.~Ward$^{41}$,
%~Z.~Was$^{4}$, ~G.~Weiglein$^{32}$, ~C.~Weiland$^{42}$, ~S.~Weinzierl$^{43}$, S.A.~Yost$^{44}$, ~J.~Zurita$^{45,46}$

%\vspace*{07mm}  %tr 14 mm

%\begin{flushleft}
%{\em\small
%{$^{1}$DPNC University of Geneva, Switzerland}
%\\
%{$^2$Institute  of Physics, University of Silesia, 40-007 Katowice, Poland}
%\\
%{$^{3}$ Faculty of Science, University of Hradec Kr\'alov\'e, Czech Republic}
%\\
%{$^4$Institute of Nuclear Physics, PAN, 
%ul. Radzikowskiego 152, 
%31-342 Krak\'ow, Poland}
%\\
%{$^{5}$CERN, CH-1211 Geneva 23, Switzerland}
%\\
%{$^{6}$Deutsches Elektronen--Synchrotron, DESY, 15738 Zeuthen, Germany}
%\\
%{$^{7}$ Center for Cosmology, Particle Physics and Phenomenology (CP3), Universit\'e Catholique de Louvain, 1348 Louvain-La-Neuve, Belgium}
%\\
%{$^{8}$ Instituto de F\'{\i}sica Corpuscular, Universitat de Val\`{e}ncia -- Consejo Superior de Investigaciones Cient\'{\i}ficas, 
%       Parc Cient\'{\i}fic, E-46980 Paterna, Valencia, Spain}
%\\
%{$^{9}$ Institut f\"ur Theoretische Physik, Eberhard Karls Universit\"at T\"ubingen, Auf der Morgenstelle 14, D-72076 T\"ubingen, Germany},
%\\
%{$^{10}$ Indian Institute of Technology, Kanpur, India}
%\\
%{$^{11}$  University of Louisville, Louisville, KY 40292 USA}
%\\
%{$^{12}$ Physik Department T31, Technische Universit\"at M\"unchen, Garching, Germany}
%\\
%{$^{13}$ Institut f{\"u}r Physik, Johannes Gutenberg-Universit{\"a}t Mainz, D-55099 Mainz, Germany},
%\\
%{$^{14}$ Department Physik, Universit\"at Siegen, Walter-Flex-Str. 3, 57068 Siegen Germany}
%\\
%{$^{15}$ Bethe Center for Theoretical Physics \& Physikalisches Institut der Universit\"at Bonn, Nu{\ss}allee 12, 53115 Bonn, Germany}
%\\
%{$^{16}$ Physikalisches Institut, Albert-Ludwigs-Universit\"at Freiburg, Hermann-Herder-Str. 3, D-79104 Freiburg, Germany}
%\\
%{$^{17}$ Physics Department, Florida State University, 77 Chieftan Way, Tallahassee, FL 32306, U.S.A.}
%\\
%{$^{18}$ Theoretical Physics Division, 
%       Department of Mathematical Sciences, University of Liverpool, P.O. Box 
%       147, Liverpool, L69 3BX, United Kingdom},
%\\
%{$^{19}$Institut f\"ur Theoretische Physik, Universit\"at Hamburg,
%       Luruper Chaussee 149, 22761 Hamburg, Germany}
%\\
%{$^{20}$ Max Planck Institute for Physics, F\"ohringer Ring 6, 80805 M\"unchen, Germany}
%\\
%{$^{21}$ Instituto de F\'isica Te\'orica (UAM/CSIC), Universidad Aut\'onoma de Madrid, Cantoblanco, 28049 Madrid, Spain}
%\\
%{$^{22}$ Instituto de F\'isica de Cantabria (CSIC-UC), 39005 Santander, Spain}
%\\
%{$^{23}$ Campus of International Excellence UAM+CSIC, Cantoblanco, 28049, Madrid, Spain}
%\\
%{$^{24}$ Humboldt--Universit\"at zu Berlin, Institut f\"ur Physik, Newtonstrasse 15, D--12489 Berlin, Germany},
%\\
%{$^{25}$Institute of Physics, University of Debrecen, 4010 Debrecen, PO Box 105, Hungary},
%\\
%{$^{26}$ Physik-Institut, Universit{\"a}t Z{\"u}rich, Winterthurerstrasse 190, 8057 Z{\"u}rich, Switzerland},
%\\
%{$^{27}$ Fakult\"at f\"ur Physik und Astronomie, Universit\"at W\"urzburg, Emil-Hilb-Weg 22, 97074 W\"urzburg Germany}
%\\
%{$^{28}$ Institut de Physique Th\'eorique, CEA, CNRS, Universit\'e Paris-Saclay, F-91191 Gif-sur-Yvette cedex, France}
%\\
%{$^{29}$ Sorbonne Universit\'e, CNRS, Laboratoire de Physique Th\'eorique et Hautes \'Energies (LPTHE), 4 Place Jussieu, 75252 Paris CEDEX 05, France}
%\\
%{$^{30}$ Marian Smoluchowski Institute of Physics, Jagiellonian University, Cracow, PL}
%\\
%{$^{31}$ Departamento de F\'{i}sica Te\'orica y del Cosmos and CAFPE, Universidad de Granada, Campus Fuentenueva s.n., E-18071 Granada, Spain}
%\\
%{$^{32}$Deutsches Elektronen--Synchrotron, DESY, Notkestra{\ss}e 85, 22607 Hamburg, Germany}
%\\
%{$^{33}$ Institute for Particle Physics Phenomenology, University of Durham, Durham DH1 3LE, UK}
%\\
%{$^{34}$ Institute for Theoretical Physics, ETH Z\"urich, Wolfgang-Pauli-Str. 27, 8093 Z\"urich, Switzerland}
%\\
%{$^{35}$ Institut f\"ur Theoretische Teilchenphysik und   
%       Kosmologie,   RWTH Aachen University, Sommerfeldstra\ss e 16,  52056 Aachen, Germany}
%\\
%{$^{36}$ MTA-DE Particle Physics Research Group, University of Debrecen, 4010 Debrecen, PO Box 105, Hungary}
%\\
%{$^{37}$ Paul Scherrer Institut, CH-5232 Villigen PSI, Switzerland}
%\\
%{$^{38}$ Department of Physics, University of Toronto, 60 St George St., Toronto, Ontario, M5S 1A7, Canada}
%\\
%{$^{39}$ Institute for Theoretical Physics, E\"otv\"os Lor\'and University, P\'azm\'any P\'eter 1/A, H-1117 Budapest, Hungary}
%\\
%{$^{40}$  School of Mathematics,
%       Trinity College Dublin, The University of Dublin, Ireland}
%\\
%{$^{41}$ Baylor University, Waco, TX, USA}
%\\
%{$^{42}$ Pittsburgh Particle physics, Astrophysics, and Cosmology Center, %Department of Physics and Astronomy, University of Pittsburgh,
% 3941 O'Hara St., Pittsburgh, PA 15260, USA}
%\\
%{$^{43}$ PRISMA Cluster of Excellence, Inst. f{\"u}r Physik, Johannes Gutenberg-Universit{\"a}t, 55099 Mainz, Germany}
%\\
%{$^{44}$ The Citadel, Charleston, SC, USA}
%\\
%{$^{45}$ Institute for Nuclear Physics (IKP), Karlsruhe Institute of Technology,
%Hermann-von-Helmholtz-Platz 1, D-76344 Eggenstein-Leopoldshafen, Germany}
%\\
%{$^{46}$ Institute for Theoretical Particle Physics (TTP), Karlsruhe Institute of Technology, Engesserstra\ss e 7, D-76128 Karlsruhe, Germany}
%}
%\end{flushleft}
%\end{center}
%\renewcommand{\footnoterule}{%
%  \kern -3pt
%  \hrule width \textwidth height 1pt
%  \kern 2pt
%}
% makes a reasonable footnote with some rule:
\kern -3pt
\hrule width 2in
\kern 2.6pt
%$^{*}$ Corresponding editor, E-mail: janusz.gluza@cern.ch.



==> Headers/authors_old.tex <==
\begin{center}
A.~Blondel$^{1}$, ~J.~Gluza\footnote{Corresponding editor, E-mail: janusz.gluza@cern.ch}$^{,2,3}$,  ~S.~Jadach$^4$, ~P.~Janot$^{5}$, ~M.~McCullough$^{5}$, ~T.~Riemann$^{2,6}$ (eds.),
\\
S.~Abreu$^{7}$, ~J.J.~Aguilera-Verdugo$^{8}$,
~A.B.~Arbuzov$^{9}$,
~J.~Baglio$^{10}$, ~S.D.~Bakshi$^{11}$, ~S.~Banerjee$^{12}$, ~C.~Bobeth$^{13}$, ~C.~Bogner$^{14}$,
~S.G.~Bondarenko$^{9}$,
~S.~Borowka$^{5}$, ~S.~Bra{\ss}$^{15}$, ~J.~Chakrabortty$^{11}$ , ~M.~Chrzaszcz$^{4}$, ~D.~d'Enterria$^{5}$,
~F.~Domingo$^{16}$, ~J.~Dormans$^{17}$,
~F.~Driencourt-Mangin$^{8}$,
~Ya.V.~Dydyshka$^{18}$,
~F.~Febres~Cordero$^{17,19}$, ~J.A.~Gracey$^{20}$, ~Zhi-Guo~He$^{21}$, ~G.~Heinrich$^{22}$, ~S.~Heinemeyer$^{23,24,25}$,
~I.~H\"onemann$^{14}$, ~H.~Ita$^{17}$, ~S.~Jahn$^{22}$, ~F.~Jegerlehner$^{6,26}$, ~S.~P.~Jones$^{5}$,
~L.V.~Kalinovskaya$^{18}$,
~A.~Kardos$^{27}$, ~M.~Kerner$^{28}$, ~W.~Kilian$^{15}$,
~S.~Kluth$^{22}$, ~B.~A.~Kniehl$^{21}$, ~A.~Maier$^{6}$, ~P.~Maierh\"ofer$^{17}$, ~T.~Ohl$^{29}$, ~B.~Page$^{30}$, ~S.~Pa{\ss}ehr$^{31}$, ~S.K.~Patra$^{11}$, ~W.~Placzek$^{32}$, ~R.~Pittau$^{33}$, ~J.~Plenter$^{8}$, ~S.~Ram\'{\i}rez-Uribe$^{8}$, 
~J.~Reuter$^{34}$, ~G.~Rodrigo$^{8}$, ~V.~Rothe$^{34}$,
~L.A.~Rumyantsev$^{18,35}$,
~R.R.~Sadykov$^{18}$,
~J.~Schlenk$^{36}$, ~G.~F.~R.~Sborlini$^{8}$, ~A.~Schweitzer$^{37}$, ~C.~Schwinn$^{38}$, ~M.~Skrzypek$^{4}$, ~G.~Somogyi$^{39}$, ~M.~Spira$^{40}$, ~P.~Stienemeier$^{34}$, ~R.~Szafron$^{13}$, 
~K.~Tempest$^{41}$, ~W.~J.~Torres Bobadilla$^{8}$, ~S.~Tracz$^{8}$, ~Z.~Tr\'ocs\'anyi$^{39,42}$, ~Z.~Tulip\'ant$^{39}$,
~J.~Usovitsch$^{43}$, ~A.~Verbytskyi$^{22}$, ~B.F.L.~Ward$^{44}$,
~Z.~Was$^{4}$, ~G.~Weiglein$^{34}$, ~C.~Weiland$^{45}$, ~S.~Weinzierl$^{46}$,
~V.L.~Yermolchyk$^{18}$
~S.A.~Yost$^{47}$, ~J.~Zurita$^{48,49}$

%72+5
%C.Grojean
%Calame,Piccinini,Montagna,Nicrosini - 2nd arxiv

\vspace*{07mm}  %tr 14 mm

\begin{flushleft}
{\em\small
{$^{1}$ DPNC University of Geneva, Switzerland}
\\
{$^2$ Institute  of Physics, University of Silesia, 40-007 Katowice, Poland}
\\
{$^{3}$ Faculty of Science, University of Hradec Kr\'alov\'e, Czech Republic}
\\
{$^4$ Institute of Nuclear Physics, PAN, 
%ul. Radzikowskiego 152, 
31-342 Krak\'ow, Poland}
\\
{$^{5}$ CERN, CH-1211 Geneva 23, Switzerland}
\\
{$^{6}$ Deutsches Elektronen--Synchrotron, DESY, 15738 Zeuthen, Germany}
\\
{$^{7}$ Center for Cosmology, Particle Physics and Phenomenology (CP3), Universit\'e Catholique de Louvain, 1348 Louvain-La-Neuve, Belgium}
\\
{$^{8}$ Instituto de F\'{\i}sica Corpuscular, Universitat de Val\`{e}ncia -- Consejo Superior de Investigaciones Cient\'{\i}ficas, 
        Parc Cient\'{\i}fic, E-46980 Paterna, Valencia, Spain}
\\
{$^{9}$ Bogoliubov Laboratory of Theoretical Physics, JINR, Dubna, 141980 Russia}
\\
{$^{10}$ Institut f\"ur Theoretische Physik, Eberhard Karls Universit\"at T\"ubingen, Auf der Morgenstelle 14, D-72076 T\"ubingen, Germany},
\\
{$^{11}$ Indian Institute of Technology, Kanpur, India}
\\
{$^{12}$  University of Louisville, Louisville, KY 40292 USA}
\\
{$^{13}$ Physik Department T31, Technische Universit\"at M\"unchen, Garching, Germany}
\\
{$^{14}$ Institut f{\"u}r Physik, Johannes Gutenberg-Universit{\"a}t Mainz, D-55099 Mainz, Germany},
\\
{$^{15}$ Department Physik, Universit\"at Siegen, Walter-Flex-Str. 3, 57068 Siegen Germany}
\\
{$^{16}$ Bethe Center for Theoretical Physics \& Physikalisches Institut der Universit\"at Bonn, Nu{\ss}allee 12, 53115 Bonn, Germany}
\\
{$^{17}$ Physikalisches Institut, Albert-Ludwigs-Universit\"at Freiburg, Hermann-Herder-Str. 3, D-79104 Freiburg, Germany}
\\
{$^{18}$  Dzhelepov Laboratory of Nuclear Problems, JINR, Dubna, 141980 Russia}
\\
{$^{19}$ Physics Department, Florida State University, 77 Chieftan Way, Tallahassee, FL 32306, U.S.A.}
\\
{$^{20}$ Theoretical Physics Division, 
        Department of Mathematical Sciences, University of Liverpool, P.O. Box 
        147, Liverpool, L69 3BX, United Kingdom},
\\
{$^{21}$Institut f\"ur Theoretische Physik, Universit\"at Hamburg,
        Luruper Chaussee 149, 22761 Hamburg, Germany}
\\
{$^{22}$ Max Planck Institute for Physics, F\"ohringer Ring 6, 80805 M\"unchen, Germany}
\\
{$^{23}$ Instituto de F\'isica Te\'orica (UAM/CSIC), Universidad Aut\'onoma de Madrid, Cantoblanco, 28049 Madrid, Spain}
\\
{$^{24}$ Instituto de F\'isica de Cantabria (CSIC-UC), 39005 Santander, Spain}
\\
{$^{25}$ Campus of International Excellence UAM+CSIC, Cantoblanco, 28049, Madrid, Spain}
\\
{$^{26}$ Humboldt--Universit\"at zu Berlin, Institut f\"ur Physik, Newtonstrasse 15, D--12489 Berlin, Germany},
\\
{$^{27}$Institute of Physics, University of Debrecen, 4010 Debrecen, PO Box 105, Hungary},
\\
{$^{28}$ Physik-Institut, Universit{\"a}t Z{\"u}rich, Winterthurerstrasse 190, 8057 Z{\"u}rich, Switzerland},
\\
{$^{29}$ Fakult\"at f\"ur Physik und Astronomie, Universit\"at W\"urzburg, Emil-Hilb-Weg 22, 97074 W\"urzburg Germany}
\\
{$^{30}$ Institut de Physique Th\'eorique, CEA, CNRS, Universit\'e Paris-Saclay, F-91191 Gif-sur-Yvette cedex, France}
\\
{$^{31}$ Sorbonne Universit\'e, CNRS, Laboratoire de Physique Th\'eorique et Hautes \'Energies (LPTHE), 4 Place Jussieu, 75252 Paris CEDEX 05, France}
\\
{$^{32}$ Marian Smoluchowski Institute of Physics, Jagiellonian University, Cracow, Poland}
\\
{$^{33}$ Departamento de F\'{i}sica Te\'orica y del Cosmos and CAFPE, Universidad de Granada, Campus Fuentenueva s.n., E-18071 Granada, Spain}
\\
{$^{34}$ Deutsches Elektronen--Synchrotron, DESY, Notkestra{\ss}e 85, 22607 Hamburg, Germany}
\\
{$^{35}$ Institute of Physics, Southern Federal University, Rostov-on-Don, 344090 Russia} 
\\
{$^{36}$ Institute for Particle Physics Phenomenology, University of Durham, Durham DH1 3LE, UK}
\\
{$^{37}$ Institute for Theoretical Physics, ETH Z\"urich, Wolfgang-Pauli-Str. 27, 8093 Z\"urich, Switzerland}
\\
{$^{38}$ Institut f\"ur Theoretische Teilchenphysik und   
        Kosmologie,   RWTH Aachen University, Sommerfeldstra\ss e 16,  52056 Aachen, Germany}
\\
{$^{39}$ MTA-DE Particle Physics Research Group, University of Debrecen, 4010 Debrecen, PO Box 105, Hungary}
\\
{$^{40}$ Paul Scherrer Institut, CH-5232 Villigen PSI, Switzerland}
\\
{$^{41}$ Department of Physics, University of Toronto, 60 St George St., Toronto, Ontario, M5S 1A7, Canada}
\\
{$^{42}$ Institute for Theoretical Physics, E\"otv\"os Lor\'and University, P\'azm\'any P\'eter 1/A, H-1117 Budapest, Hungary}
\\
{$^{43}$  School of Mathematics,
        Trinity College Dublin, The University of Dublin, Ireland}
\\
{$^{44}$ Baylor University, Waco, TX, USA}
\\
{$^{45}$ Pittsburgh Particle physics, Astrophysics, and Cosmology Center, Department of Physics and Astronomy, University of Pittsburgh,
 3941 O'Hara St., Pittsburgh, PA 15260, USA}
\\
{$^{46}$ PRISMA Cluster of Excellence, Inst. f{\"u}r Physik, Johannes Gutenberg-Universit{\"a}t, 55099 Mainz, Germany}
\\
{$^{47}$ The Citadel, Charleston, SC, USA}
\\
{$^{48}$ Institute for Nuclear Physics (IKP), Karlsruhe Institute of Technology,
  Hermann-von-Helmholtz-Platz 1, D-76344 Eggenstein-Leopoldshafen, Germany}
\\
{$^{49}$ Institute for Theoretical Particle Physics (TTP), Karlsruhe Institute of Technology, Engesserstra\ss e 7, D-76128 Karlsruhe, Germany}
}
\end{flushleft}
\end{center}

%before sanc authors
%\begin{center}
%A.~Blondel$^{1}$, ~J.~Gluza\footnote{Corresponding editor, E-mail: janusz.gluza@cern.ch}$^{,2,3}$,  ~S.~Jadach$^4$, ~P.~Janot$^{5}$, ~M.~McCullough$^{5}$, ~T.~Riemann$^{2,6}$ (eds.),
%\\
%S.~Abreu$^{7}$, ~J.J.~Aguilera-Verdugo$^{8}$, ~J.~Baglio$^{9}$, ~S.D.~Bakshi$^{10}$, ~S.~Banerjee$^{11}$, ~C.~Bobeth$^{12}$, ~C.~Bogner$^{13}$, ~S.~Borowka$^{5}$, ~S.~Bra{\ss}$^{14}$, ~J.~Chakrabortty$^{10}$ , ~M.~Chrzaszcz$^4$, ~F.~Domingo$^{15}$, ~J.~Dormans$^{16}$, ~F.~Driencourt-Mangin$^{8}$, ~F.~Febres~Cordero$^{16,17}$, ~J.A.~Gracey$^{18}$, ~Zhi-Guo~He$^{19}$, ~G.~Heinrich$^{20}$, ~S.~Heinemeyer$^{21,22,23}$,
%~I.~H\"onemann$^{13}$, ~H.~Ita$^{16}$, ~S.~Jahn$^{20}$, ~F.~Jegerlehner$^{6,24}$, ~S.~P.~Jones$^{5}$, ~A.~Kardos$^{25}$, ~M.~Kerner$^{26}$, ~W.~Kilian$^{14}$,
%~S.~Kluth$^{20}$, ~B.~A.~Kniehl$^{19}$, ~A.~Maier$^{6}$, ~P.~Maierh\"ofer$^{16}$, ~T.~Ohl$^{27}$, ~B.~Page$^{28}$, ~S.~Pa{\ss}ehr$^{29}$, ~S.K.~Patra$^{10}$, ~W.~Placzek$^{30}$, ~R.~Pittau$^{31}$, ~J.~Plenter$^{8}$, ~S.~Ram\'{\i}rez-Uribe$^{8}$, 
%~J.~Reuter$^{32}$, ~G.~Rodrigo$^{8}$, ~V.~Rothe$^{32}$, ~J.~Schlenk$^{33}$, ~G.~F.~R.~Sborlini$^{8}$, ~A.~Schweitzer$^{34}$, ~C.~Schwinn$^{35}$, ~M.~Skrzypek$^{4}$, ~G.~Somogyi$^{36}$, ~M.~Spira$^{37}$, ~P.~Stienemeier$^{32}$, ~R.~Szafron$^{12}$, 
%~K.~Tempest$^{38}$, ~W.~J.~Torres Bobadilla$^{8}$, ~S.~Tracz$^{8}$, ~Z.~Tr\'ocs\'anyi$^{37,39}$, ~Z.~Tulip\'ant$^{36}$,
%~J.~Usovitsch$^{40}$, ~A.~Verbytskyi$^{20}$, ~B.F.L.~Ward$^{41}$,
%~Z.~Was$^{4}$, ~G.~Weiglein$^{32}$, ~C.~Weiland$^{42}$, ~S.~Weinzierl$^{43}$, S.A.~Yost$^{44}$, ~J.~Zurita$^{45,46}$

%\vspace*{07mm}  %tr 14 mm

%\begin{flushleft}
%{\em\small
%{$^{1}$DPNC University of Geneva, Switzerland}
%\\
%{$^2$Institute  of Physics, University of Silesia, 40-007 Katowice, Poland}
%\\
%{$^{3}$ Faculty of Science, University of Hradec Kr\'alov\'e, Czech Republic}
%\\
%{$^4$Institute of Nuclear Physics, PAN, 
%ul. Radzikowskiego 152, 
%31-342 Krak\'ow, Poland}
%\\
%{$^{5}$CERN, CH-1211 Geneva 23, Switzerland}
%\\
%{$^{6}$Deutsches Elektronen--Synchrotron, DESY, 15738 Zeuthen, Germany}
%\\
%{$^{7}$ Center for Cosmology, Particle Physics and Phenomenology (CP3), Universit\'e Catholique de Louvain, 1348 Louvain-La-Neuve, Belgium}
%\\
%{$^{8}$ Instituto de F\'{\i}sica Corpuscular, Universitat de Val\`{e}ncia -- Consejo Superior de Investigaciones Cient\'{\i}ficas, 
%	Parc Cient\'{\i}fic, E-46980 Paterna, Valencia, Spain}
%\\
%{$^{9}$ Institut f\"ur Theoretische Physik, Eberhard Karls Universit\"at T\"ubingen, Auf der Morgenstelle 14, D-72076 T\"ubingen, Germany},
%\\
%{$^{10}$ Indian Institute of Technology, Kanpur, India}
%\\
%{$^{11}$  University of Louisville, Louisville, KY 40292 USA}
%\\
%{$^{12}$ Physik Department T31, Technische Universit\"at M\"unchen, Garching, Germany}
%\\
%{$^{13}$ Institut f{\"u}r Physik, Johannes Gutenberg-Universit{\"a}t Mainz, D-55099 Mainz, Germany},
%\\
%{$^{14}$ Department Physik, Universit\"at Siegen, Walter-Flex-Str. 3, 57068 Siegen Germany}
%\\
%{$^{15}$ Bethe Center for Theoretical Physics \& Physikalisches Institut der Universit\"at Bonn, Nu{\ss}allee 12, 53115 Bonn, Germany}
%\\
%{$^{16}$ Physikalisches Institut, Albert-Ludwigs-Universit\"at Freiburg, Hermann-Herder-Str. 3, D-79104 Freiburg, Germany}
%\\
%{$^{17}$ Physics Department, Florida State University, 77 Chieftan Way, Tallahassee, FL 32306, U.S.A.}
%\\
%{$^{18}$ Theoretical Physics Division, 
%	Department of Mathematical Sciences, University of Liverpool, P.O. Box 
%	147, Liverpool, L69 3BX, United Kingdom},
%\\
%{$^{19}$Institut f\"ur Theoretische Physik, Universit\"at Hamburg,
%	Luruper Chaussee 149, 22761 Hamburg, Germany}
%\\
%{$^{20}$ Max Planck Institute for Physics, F\"ohringer Ring 6, 80805 M\"unchen, Germany}
%\\
%{$^{21}$ Instituto de F\'isica Te\'orica (UAM/CSIC), Universidad Aut\'onoma de Madrid, Cantoblanco, 28049 Madrid, Spain}
%\\
%{$^{22}$ Instituto de F\'isica de Cantabria (CSIC-UC), 39005 Santander, Spain}
%\\
%{$^{23}$ Campus of International Excellence UAM+CSIC, Cantoblanco, 28049, Madrid, Spain}
%\\
%{$^{24}$ Humboldt--Universit\"at zu Berlin, Institut f\"ur Physik, Newtonstrasse 15, D--12489 Berlin, Germany},
%\\
%{$^{25}$Institute of Physics, University of Debrecen, 4010 Debrecen, PO Box 105, Hungary},
%\\
%{$^{26}$ Physik-Institut, Universit{\"a}t Z{\"u}rich, Winterthurerstrasse 190, 8057 Z{\"u}rich, Switzerland},
%\\
%{$^{27}$ Fakult\"at f\"ur Physik und Astronomie, Universit\"at W\"urzburg, Emil-Hilb-Weg 22, 97074 W\"urzburg Germany}
%\\
%{$^{28}$ Institut de Physique Th\'eorique, CEA, CNRS, Universit\'e Paris-Saclay, F-91191 Gif-sur-Yvette cedex, France}
%\\
%{$^{29}$ Sorbonne Universit\'e, CNRS, Laboratoire de Physique Th\'eorique et Hautes \'Energies (LPTHE), 4 Place Jussieu, 75252 Paris CEDEX 05, France}
%\\
%{$^{30}$ Marian Smoluchowski Institute of Physics, Jagiellonian University, Cracow, PL}
%\\
%{$^{31}$ Departamento de F\'{i}sica Te\'orica y del Cosmos and CAFPE, Universidad de Granada, Campus Fuentenueva s.n., E-18071 Granada, Spain}
%\\
%{$^{32}$Deutsches Elektronen--Synchrotron, DESY, Notkestra{\ss}e 85, 22607 Hamburg, Germany}
%\\
%{$^{33}$ Institute for Particle Physics Phenomenology, University of Durham, Durham DH1 3LE, UK}
%\\
%{$^{34}$ Institute for Theoretical Physics, ETH Z\"urich, Wolfgang-Pauli-Str. 27, 8093 Z\"urich, Switzerland}
%\\
%{$^{35}$ Institut f\"ur Theoretische Teilchenphysik und   
%	Kosmologie,   RWTH Aachen University, Sommerfeldstra\ss e 16,  52056 Aachen, Germany}
%\\
%{$^{36}$ MTA-DE Particle Physics Research Group, University of Debrecen, 4010 Debrecen, PO Box 105, Hungary}
%\\
%{$^{37}$ Paul Scherrer Institut, CH-5232 Villigen PSI, Switzerland}
%\\
%{$^{38}$ Department of Physics, University of Toronto, 60 St George St., Toronto, Ontario, M5S 1A7, Canada}
%\\
%{$^{39}$ Institute for Theoretical Physics, E\"otv\"os Lor\'and University, P\'azm\'any P\'eter 1/A, H-1117 Budapest, Hungary}
%\\
%{$^{40}$  School of Mathematics,
%	Trinity College Dublin, The University of Dublin, Ireland}
%\\
%{$^{41}$ Baylor University, Waco, TX, USA}
%\\
%{$^{42}$ Pittsburgh Particle physics, Astrophysics, and Cosmology Center, %Department of Physics and Astronomy, University of Pittsburgh,
% 3941 O'Hara St., Pittsburgh, PA 15260, USA}
%\\
%{$^{43}$ PRISMA Cluster of Excellence, Inst. f{\"u}r Physik, Johannes Gutenberg-Universit{\"a}t, 55099 Mainz, Germany}
%\\
%{$^{44}$ The Citadel, Charleston, SC, USA}
%\\
%{$^{45}$ Institute for Nuclear Physics (IKP), Karlsruhe Institute of Technology,
%Hermann-von-Helmholtz-Platz 1, D-76344 Eggenstein-Leopoldshafen, Germany}
%\\
%{$^{46}$ Institute for Theoretical Particle Physics (TTP), Karlsruhe Institute of Technology, Engesserstra\ss e 7, D-76128 Karlsruhe, Germany}
%}
%\end{flushleft}
%\end{center}
%\renewcommand{\footnoterule}{%
%  \kern -3pt
%  \hrule width \textwidth height 1pt
%  \kern 2pt
%}
% makes a reasonable footnote with some rule:
\kern -3pt
\hrule width 2in
\kern 2.6pt
%$^{*}$ Corresponding editor, E-mail: janusz.gluza@cern.ch.



==> Macros/definitions.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%% SM notation %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newcommand{\bhlumi}{{\tt BHLUMI}}
%\newcommand{\bhwide}{{\tt BHWIDE}}
%\newcommand{\babayaga}{{\tt BabaYaga}}
\newcommand{\order}[1]{${\cal O}(#1)$}
\newcommand{\KK}{${\cal KK}$}
\def\Ordex#1{${\cal O}(#1)_{exp}$}
\def\Order#1{${\cal O}(#1)$}
\def\OrderLL#1{${\cal O}(#1)_{\rm LL}$}
\def\bbeta{\bar{\beta}}
\newcommand{\sfac}{\mathfrak{s}}
\def\hbeta{\hat{\beta}}
  
%sven
\newcommand{\AmpE}[2]{{\cal A}^{{\rm #1}}_{#2}}
\newcommand{\Amp}[3]{{\cal A}^{{\rm #1}}_{#2}\ifthenelse{\isempty{#3}}{}{{[#3]}}}
\newcommand{\tAmp}[3]{\tilde{\cal A}^{{\rm #1}}_{#2}\ifthenelse{\isempty{#3}}{}{{[#3]}}}
\newcommand{\cp}{\ensuremath{{\cal CP}}}
\newcommand{\IE}{i.e.\ }
\newcommand{\EG}{e.g.\ }
\newcommand{\FH}{\texttt{FeynHiggs}}
\newcommand{\I}{\mathrm{i}}
\newcommand{\Un}[1]{(U_n)_{#1}}
\newcommand{\Anull}[1]{A_{0}{\left(#1\right)}}
\newcommand{\Bnull}[1]{B_{0}{\left(#1\right)}}
\newcommand{\Cnull}[1]{C_{0}{\left(#1\right)}}
\newcommand{\Beins}[1]{B_{1}{\left(#1\right)}}
\newcommand{\Bnnull}[1]{B_{00}{\left(#1\right)}}
\newcommand{\DBnull}[1]{B_{0}^{\prime}{\left(#1\right)}}
\newcommand{\mueff}{\mu_{\rm eff}}
\newcommand{\DRbar}{\ensuremath{\overline{\mathrm{DR}}}}
\newcommand{\MSbar}{\ensuremath{\overline{\mathrm{MS}}}}
\newcommand{\OS}{\ensuremath{\mathrm{OS}}}
\newcommand{\simord}{\sim}
\newcommand{\gsim}{\gtrsim}


%\renewcommand{\refname}{References.}
\renewcommand{\theequation}{\thesection.\arabic{equation}} 
\def\thefootnote{\fnsymbol{footnote}} 
\newcommand{\sect}[1]{ \section{#1} \setcounter{equation}{0} } 

\newcommand{\half}{\mbox{\small{$\frac{1}{2}$}}} 
\newcommand{\third}{\mbox{\small{$\frac{1}{3}$}}} 
\newcommand{\quarter}{\mbox{\small{$\frac{1}{4}$}}} 
%\newcommand{\MSbar}{\overline{\mbox{MS}}} 
\newcommand{\Nc}{N_{\!c}}
\newcommand{\kslash}{k \! \! \! /}
\newcommand{\pslash}{p \! \! \! /}
\newcommand{\qslash}{q \! \! \! /}
\newcommand{\partialslash}{\partial \! \! \! /}
\newcommand{\xslash}{x \! \! \! /}
\newcommand{\yslash}{y \! \! \! /}
\newcommand{\zslash}{z \! \! \! /}


\providecommand{\gaga}{\gamma\,\gamma}
\providecommand{\epem}{\rm e^{+}e^{-}}
\providecommand{\alphas}{\alpha_{\rm s}}
%\newcommand{\Lumi}{\mathcal{L}}
%\newcommand{\Lunits}{cm$^{-2}$s$^{-1}$}
%\newcommand{\sqrts}{\sqrt{s}}
%\newcommand{\ttbar}{t\overline{t}}

%\newcommand{\Lumi}{\mathcal{L}}
\newcommand{\Lunits}{cm$^{-2}$s$^{-1}$}
\newcommand{\sqrts}{\sqrt{s}}
\newcommand{\ttbar}{t\overline{t}}

\def\mathswitch#1{\relax\ifmmode#1\else$#1$\fi}
\def\mathswitchr#1{\relax\ifmmode{\mathrm{#1}}\else$\mathrm{#1}$\fi}

\newcommand{\Pt}{\mathswitchr t}
\def \sd {\texttt{SD}{}}
\def\order#1{\ensuremath{{\cal O}(#1)}}

\newcommand{\bhlumi}{{\tt BHLUMI}}
\newcommand{\sanc}{{\tt SANC}}

\newcommand{\veps}{{\varepsilon}}

\newcommand{\afb}{{A_{FB}}}
\newcommand{\vmax}{{v_{\max}}}
\newcommand{\cst}{{\triangle}}
\newcommand{\Pmf}{\mathfrak{P}}
\newcommand{\Dmf}{\mathfrak{D}}
\newcommand{\Bmf}{\mathfrak{B}}
\newcommand{\Emf}{\mathfrak{E}}
\newcommand{\Rmf}{\mathfrak{R}}
\newcommand{\Zmf}{\mathfrak{Z}}
\newcommand{\Mmf}{\mathfrak{M}}

\newcommand{\MW}{\mathswitch {M_{\PW}}}
\newcommand{\MZ}{\mathswitch {M_{\PZ}}}
\newcommand{\GZ}{\mathswitch {\Gamma_{\PZ}}}
\newcommand{\MH}{\mathswitch {M_{\PH}}}
\newcommand{\MA}{\mathswitch {M_{\PA}}}
\newcommand{\me}{\mathswitch {m_{\Pe}}}
\newcommand{\mb}{\mathswitch {m_{\Pb}}}
\newcommand{\mt}{\mathswitch {m_{\Pt}}}
\newcommand{\mf}{m_f}
\newcommand{\scrs}{\scriptscriptstyle}
\newcommand{\sw}{\mathswitch {s_{\scrs\PW}}}
\newcommand{\cw}{\mathswitch {c_{\scrs\PW}}}
\newcommand{\mw}{\mathswitch {\overline{M}_\PW}} 
\newcommand{\mz}{\mathswitch {\overline{M}_\PZ}}
\newcommand{\gw}{\mathswitch {\overline{\Gamma}_{\PW}}}
\newcommand{\gz}{\mathswitch {\overline{\Gamma}_{\PZ}}}
\newcommand{\as}{\alpha_{\mathrm s}}
\newcommand{\at}{\alpha_\Pt}
\newcommand{\seff}[1]{\sin^2\theta_{\rm eff}^{\rm #1}}



%%%%%%%%%%%%%%%%%%%%%%%% other notation %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\tev}{\,\, \mathrm{TeV}}
\newcommand{\gev}{\,\, \mathrm{GeV}}
\newcommand{\mev}{\,\, \mathrm{MeV}}
\newcommand{\re}{\Re e \,}
\newcommand{\im}{\Im m \,}
\newcommand{\dd}{\partial}
\newcommand{\OO}{{\mathcal O}}
\newcommand{\anc}{\rule{0mm}{0mm}}

%%%%%%%%%%%%%%%%%%%%%%%% other notation %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\bracket}[1]{{\left\langle #1 \right\rangle}}

\DeclareMathOperator{\Pexp}{Pexp}
\DeclareMathOperator{\Ima}{Im}
\DeclareMathOperator{\coIma}{coIm}
\DeclareMathOperator{\rank}{rank}

\newcommand{\nn}{\nonumber}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%% JB %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Li}{{\rm Li}}
\newcommand{\HA}{{\rm H}}
\newcommand{\HT}{{\rm H}^*}
\newcommand{\Mvec}{{\rm\bf M}}
\newcommand{\ep}{\varepsilon}
\newcommand{\shuffle}{\,\raisebox{1.2ex}[0mm][0mm]{\rotatebox{270}{$\exists$}} \,}
\newcommand{\SigmaP}{\texttt{Sigma}}

%%%%%%%%%%%%%%%%%%%%%%%%%% MBnum %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand*{\CO}{\mathcal{O}}
\newcommand*{\CI}{\mathcal{I}}	
\newcommand*{\R}{\mathbb{R}}      % reelle Zahlen
\newcommand*{\C}{\mathbb{C}}      % komplexe Zahlen
\newcommand*{\CU}{\mathcal{U}}
\newcommand*{\CF}{\mathcal{F}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\MBresolve{{\textsf{MBresolve.m\/}}}
\def \mbnum      {\texttt{MBnumerics}{}}
\def \mbn      {\texttt{MBnumerics.m}{}}

\def \ar {\texttt{AMBRE}{}}
\def \la {\texttt{LA}{}}
\def \ga {\texttt{GA}{}}
\def \mb {\texttt{MB}{}}
\def \pltest      {\texttt{PlanarityTest}{}}
\def \mbn      {\texttt{MBnumerics.m}{}}
\def \ambre   {\texttt{AMBRE~}{}}
\def \ambrenp {\texttt{AMBRE\_np~}{}}
\def \mbsums  {\texttt{MBsums~}{}}
\def \math {\texttt{Mathematica}{}}
\def \mbm  {\texttt{MB.m}{}}
\def \mbr  {\texttt{MB}{}}

%%%%%%%%%%%%%%%%%%%%%%%% Usovitsch

\newcommand*{\kira}{\texttt{Kira}}
\newcommand*{\pyred}{\texttt{pyRed}}
\newcommand*{\firefly}{\texttt{FireFly}}
\newcommand*{\firesix}{\texttt{FIRE\,6}}
\newcommand*{\fermat}{\texttt{Fermat}}

%%%%%%%%%%%%%%%%%%%%%%%% Weinzierl %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}

%%%%%%%%%%%%%%%%%%%%%%%% Pittau
\newcommand{\nl}{\nonumber \\ }
\newcommand{\Eqn}[1]{Eq.~(\ref{#1})}
\newcommand{\Fign}[1]{Fig.~\ref{#1}}
\newcommand{\Secn}[1]{Sec.~\ref{#1}}

%%%%% Hcuba
\newcommand\Vol{\mathop{\mathrm{Vol}}}
\newcommand\op[1]{\mathbf{#1}}
\newcommand\opI{\op{I}}
\newcommand\opQ{\op{C}}
\newcommand\opM{\op{M}}
\newcommand\opN{\op{N}}
\newcommand\rd{\mathrm{d}}

\newcommand\reth{\mathrm{e}}
\newcommand\ri{\mathrm{i}}
%\newcommand\eg{e.g.\ }
%\newcommand\ie{i.e.\ }
\newcommand\Itot{I_{\mathrm{tot}}}
\newcommand\Etot{E_{\mathrm{tot}}}
\newcommand\epsrel{\varepsilon_{\mathrm{rel}}}
\newcommand\epsabs{\varepsilon_{\mathrm{abs}}}
\newcommand\ord{\mathcal{O}}
\newcommand\Code[1]{\ensuremath{\texttt{#1}}}
\newcommand\Var[1]{\ensuremath{\mathit{#1}}}
\newcommand\accel{_{\mathrm{accel}}}
\newcommand\cores{_{\mathrm{cores}}}



\newcommand{\babayagaNLO}{\texttt{{BabaYaga@NLO}}}
\newcommand{\babayaga}{\texttt{{BabaYaga}}}
\newcommand{\bhwide}{\texttt{{Bhwide}}}

%SANC
\newcommand{\sss}[1]{\scriptscriptstyle{#1}}
\newcommand{\ds }{\displaystyle}
\newcommand{\vpa}[2]{\sigma_{#1}^{#2}}
\newcommand{\vma}[2]{\delta_{#1}^{#2}}
\newcommand{\nll}{\nonumber\\}

\newcommand{\cpl}{c_+}
\newcommand{\cmi}{c_-}




==> Summary/acknowledgements.tex <==
%\vspace{10mm} \noindent
%{\bf\Large Acknowledgments}

\vspace{2mm}\noindent
 
Results by \textit{A.~Arbuzov, S.~Bondarenko, Ya.~Dydyshka, L.~Kalinovskaya, L.~Rumyantsev, R.~Sadykov, V.~Yermolchyk} are obtained in
the framework of state’s task N 3.9696.2017/8.9 of the Ministry of Education and Science of Russia.
\\
The work of \textit{J.~Baglio} is supported by the Institutional Strategy of the University of T\"ubingen (DFG, ZUK 63) and the Carl-Zeiss foundation. \textit{C.~Weiland} received financial support from the European Research Council under the European Union's Seventh Framework Programme (FP/2007-2013)/ERC Grant NuMass Agreement No. 617143, and he is also supported in part by the U.S. Department of Energy under contract DE-FG02-95ER40896 and in part by the PITT PACC. Their work has been done in collaboration with S. Pascoli.
\\
{\textit{S.D.~Bakshi}} acknowledges the financial support by IIT Kanpur and 
an
Arepalli-Karumuri travel grant for attending
this conference at CERN.
\\
\textit{S.~Borowka} gratefully acknowledges financial support by the ERC Starting Grant ``MathAm'' (39568).
\\
The work of \textit{J.~Chakrabortty} is supported by the Department of Science and
Technology, Government of India, under the Grant IFA12/PH/34 (INSPIRE Faculty Award),  
the Science and Engineering Research Board, Government of India, under the agreement
SERB/PHY/2016348 (Early Career Research Award), and
by a Initiation Research Grant, agreement no. IITK/PHY/2015077 of IIT Kanpur.
\\
The work of \textit{J.~Gluza} is supported in part by the Polish National Science Centre, grant number 2017/25/B/ST2/01987 and by international mobilities for research activities of the University of Hradec Kr\'alov\'e, CZ.02.2.69/0.0/0.0/16\_027/0008487.
\\
The work of \textit{J.A.~Gracey} was supported by a DFG Mercator Fellowship.
\\
The work of \textit{S.~Heinemeyer} is supported
in part by the MEINCOP Spain under contract
FPA2016-78022-P, in part by the Spanish Agencia
Estatal de Investigacion (AEI) and the EU
Fondo Europeo de Desarrollo Regional (FEDER)
through the project FPA2016-78645-P, in part by
the AEI through the grant IFT Centro de Excelencia
Severo Ochoa SEV-2016-0597, and by the
"Spanish Red Consolider Multidark" FPA2017-
90566-REDC.
\\
The work of \textit{M.~Chrzaszcz, Z.~Was} and \textit{J.~Zaremba} is partly supported by the Polish National Science Center grant 2016/23/B/ST2/03927
 and the CERN FCC Design Study Programme.
\\
The work of \textit{S.~Jadach, M.~Skrzypek} and \textit{Z.~Was} is partly supported by the Polish National Science Center grant 2016/23/B/ST2/03927
and the CERN FCC Design Study Programme.
\\
 \textit{A.~Kardos} acknowledges financial support from the Premium Postdoctoral Fellowship
program of the Hungarian Academy of Sciences. This work was supported by grant 
K 125105 of the National Research, Development and Innovation Fund in Hungary.
\\
\textit{M.~Kerner} acknowledges supported by the Swiss National Science Foundation (SNF) under grant number 200020-175595
\\
\textit{P.~Maierh\"ofer} acknowledges support by the state of Baden-W\"urttemberg through bwHPC and
the German Research Foundation (DFG) through grant no. INST 39/963-1 FUGG.
\\
The work of \textit{J.J.~Aguilera-Verdugo, F.~Driencourt-Mangin, J.~Plenter, S.~Ram\'{\i}rez-Uribe, G.~Rodrigo, G.F.R.~Sborlini, W.J.~Torres Bobadilla} and {\it S. Tracz} was supported by the Spanish Government (Agencia Estatal de Investigacion) and ERDF funds from European Commission (Grants No. FPA2017-84445-P and SEV-2014-0398), by Generalitat Valenciana (Grant No. PROMETEO/2017/053) and by Consejo Superior de Investigaciones Cient\'ificas (Grant No. PIE-201750E021).
\textit{J.~Plenter} acknowledges support from 
the "la Caixa" Foundation (ID 100010434, LCF/BQ/IN17/11620037), and from the European Union's H2020-MSCA 
Grant Agreement No. 713673, 
SR from CONACYT, 
\textit{J.J.~Aguilera-Verdugo} from Generalitat Valenciana (GRISOLIAP/2018/101)
and \textit{W.J.~Torres Bobadilla} from the Spanish Government (FJCI-2017-32128). 
\\
The work of \textit{R.~Pittau}\ was supported by the MECD project FPA2016-78220-C3-3-P.
\\ 
The work of \textit{T.~Riemann} is 
funded by Deutsche Rentenversicherung Bund. He is 
supported in part by a 2015 Alexander von Humboldt Honorary Research Scholarship of the Foundation for Polish Sciences (FNP) 
and by the Polish National Science Centre (NCN) under the Grant Agreement 
2017/25/B/ST2/01987.
Support of participation at the workshop from the FCC group is acknowledged. 
\\
The work of \textit{M.~Beneke, C.~Bobeth and R.~Szafron}\ was supported by the DFG Son\-derfor\-schung\-sbereich/Transregio 110 “Symmetries and the Emergence of Structure in QCD”.
\\
The research of \textit{J.~Schlenk} was supported by the European Union through the ERC Advanced Grant MC@NNLO (340983).
\\
{\textit{C.~Schwinn}} acknowledges support by the Heisenberg Programme of the DFG and a fellowship of the Collaborative Research Centre SFB 676 „Particles, Strings, and the Early Universe“ at Hamburg University. \\
\textit{J.~Usovitsch} has received funding from the European Research Council (ERC) under
the European Union's Horizon 2020 research and innovation programme under grant
agreement No 647356 (CutLoops).
\\
The report was partly supported by COST (European Cooperation in Science and Technology) Action CA16201 PARTICLEFACE and the CERN FCC design study programme.





